Bottom-up approach to scalable growth of molecules capable of optical cycling

Gas-phase molecules capable of repeatable, narrow-band spontaneous photon scattering are prized for direct laser cooling and quantum state detection. Recently, large molecules incorporating phenyl rings have been shown to exhibit similar vibrational closure to the small molecules demonstrated so far, and it is not yet known if the high vibrational-mode density of even larger species will eventually compromise optical cycling. Here, we systematically increase the size of hydrocarbon ligands attached to single alkaline-earth-phenoxides from (-H) to -C$_{14}$H$_{19}$ while measuring the vibrational branching fractions of the optical transition. We find that varying the ligand size from 1 to more than 30 atoms does not systematically reduce the cycle closure, which remains around 90%. Theoretical extensions to larger diamondoids and bulk diamond surface suggest that alkaline earth phenoxides may maintain the desirable scattering behavior as the system size grows further, with no indication of an upper limit.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
